Two-loop splitting in double parton distributions

Double parton distributions (DPDs) receive a short-distance contribution from a single parton splitting to yield the two observed partons. We investigate this mechanism at next-to-leading order (NLO) in perturbation theory. Technically, we compute the two-loop matching of both the position and momentum space DPDs onto ordinary PDFs. This also yields the 1 -> 2 splitting functions appearing in the evolution of momentum-space DPDs at NLO. We give results for the unpolarised, colour-singlet DPDs in all partonic channels. These quantities are required for calculations of double parton scattering at full NLO. We discuss various kinematic limits of our results, and we verify that the 1 -> 2 splitting functions are consistent with the number and momentum sum rules for DPDs.

==> equation.tex <==
\begin{alignat}{3}
  \int d x_{2}\;
  P_{qq,q}^{(1)\, v}
  &=
  \int d x_{2}\;
  P_{q\bar{q},q}^{(1)\, v} \,,
  &&
  \nonumber \\
  &
  \phantom{ = } \;\ms
  \int d x_{2}\;
    P_{\bar{q}q,q}^{(1)\, v}
  &&=
  2\, P_{\bar{q}q}^{V\,(1)} \,,
  \nonumber \\
  \int d x_{2}\;
  P_{q'\!q,q}^{(1)}
  &=
  \int d x_{2}\;
  P_{q'\!\bar{q}'\!,q}^{(1)}
  &&=
  P_{qq}^{S\,(1)}\,.
\end{alignat}

